Revisiting Shadow Detection: A New Benchmark Dataset for Complex World

Shadow detection in general photos is a nontrivial problem, due to the complexity of the real world. Though recent shadow detectors have already achieved remarkable performance on various benchmark data, their performance is still limited for general real-world situations. In this work, we collected shadow images for multiple scenarios and compiled a new dataset of 10,500 shadow images, each with labeled ground-truth mask, for supporting shadow detection in the complex world. Our dataset covers a rich variety of scene categories, with diverse shadow sizes, locations, contrasts, and types. Further, we comprehensively analyze the complexity of the dataset, present a fast shadow detection network with a detail enhancement module to harvest shadow details, and demonstrate the effectiveness of our method to detect shadows in general situations.

==> figs/shadow_area.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% dataset_area
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[tp]
	\centering
	\vspace*{0.5mm}
	\begin{subfigure}{0.195\textwidth} %0.138\textwidth; 0.195\textwidth 0.16\textwidth
		\includegraphics[width=\textwidth]{./figs/dataset_analysis/ISTD_ratio.png}
		\vspace{-5.5mm} \caption*{{\footnotesize (a) ISTD dataset: 18.58\%  }}
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
		\includegraphics[width=\textwidth]{./figs/dataset_analysis/CUHK_ratio.png}
		\vspace{-5.5mm} \caption*{{\footnotesize (c) Our dataset (overall): 39.88\%}} 
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
		\includegraphics[width=\textwidth]{./figs/dataset_analysis/ADE_ratio.png}
		\vspace{-5.5mm} \caption*{{\footnotesize 
			(d)	Shadow-ADE: 39.28\%}}
	\end{subfigure}
 \\
	\begin{subfigure}{0.195\textwidth}
		\includegraphics[width=\textwidth]{./figs/dataset_analysis/SBU_ratio.png}
		\vspace{-5.5mm} \caption*{{\footnotesize (b) SBU dataset: 17.88\%  }} 
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
		\includegraphics[width=\textwidth]{./figs/dataset_analysis/KITTI_ratio.png}
		\vspace{-5.5mm} \caption*{{\footnotesize (e) Shadow-KITTI: 51.49\%}}
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
		\includegraphics[width=\textwidth]{./figs/dataset_analysis/MAP_ratio.png}
		\vspace{-5.5mm} \caption*{{\footnotesize (f) Shadow-MAP: 43.38\%}}
	\end{subfigure}
\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=\textwidth]{./figs/dataset_analysis/USR_ratio.png}
	\vspace{-5.5mm} \caption*{{\footnotesize (g) Shadow-USR: 25.61\%}}
\end{subfigure}
\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=\textwidth]{./figs/dataset_analysis/MAP_ratio.png}
	\vspace{-5.5mm} \caption*{{\footnotesize (h) Shadow-MAP: 39.01\%}}
\end{subfigure}
	
	\vspace{-2mm}
	\caption{Shadow area distribution analysis. We report the ratio between the shadow regions and the whole images in our complex shadow dataset, ISTD dataset~\cite{wang2018stacked}, and SBU dataset~\cite{hou2019large, vicente2016noisy, vicente2016large}. The average ratio of the whole dataset is reported in each subcaption.}
	\label{fig:shadow_area}
	\vspace{-1mm}
\end{figure*}



%\begin{figure*}[tp]
%	\centering
%	\vspace*{0.5mm}
%	\begin{subfigure}{0.24\textwidth} %0.138\textwidth; 0.195\textwidth 0.16\textwidth
%		\includegraphics[width=\textwidth]{./figs/dataset_analysis/ISTD_ratio.png}
%		\vspace{-5.5mm} \caption*{{\footnotesize (a) ISTD dataset: 18.58\%  }}
%	\end{subfigure}
%	\begin{subfigure}{0.24\textwidth}
%		\includegraphics[width=\textwidth]{./figs/dataset_analysis/SBU_ratio.png}
%		\vspace{-5.5mm} \caption*{{\footnotesize (b) SBU dataset: 17.88\%  }} 
%	\end{subfigure}
%	\begin{subfigure}{0.24\textwidth}
%		\includegraphics[width=\textwidth]{./figs/dataset_analysis/CUHK_ratio.png}
%		\vspace{-5.5mm} \caption*{{\footnotesize (c) Our dataset (overall): 39.88\%}} 
%	\end{subfigure}
%	\begin{subfigure}{0.24\textwidth}
%		\includegraphics[width=\textwidth]{./figs/dataset_analysis/ADE_ratio.png}
%		\vspace{-5.5mm} \caption*{{\footnotesize 
%			(d)	Shadow-ADE: 39.28\%}}
%	\end{subfigure}
% \\
%	\begin{subfigure}{0.24\textwidth}
%		\includegraphics[width=\textwidth]{./figs/dataset_analysis/KITTI_ratio.png}
%		\vspace{-5.5mm} \caption*{{\footnotesize (e) Shadow-KITTI: 51.49\%}}
%	\end{subfigure}
%	\begin{subfigure}{0.24\textwidth}
%		\includegraphics[width=\textwidth]{./figs/dataset_analysis/MAP_ratio.png}
%		\vspace{-5.5mm} \caption*{{\footnotesize (f) Shadow-MAP: 43.38\%}}
%	\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%	\includegraphics[width=\textwidth]{./figs/dataset_analysis/USR_ratio.png}
%	\vspace{-5.5mm} \caption*{{\footnotesize (g) Shadow-USR: 25.61\%}}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%	\includegraphics[width=\textwidth]{./figs/dataset_analysis/MAP_ratio.png}
%	\vspace{-5.5mm} \caption*{{\footnotesize (h) Shadow-MAP: 39.01\%}}
%\end{subfigure}
%	
%	\vspace{-2mm}
%	\caption{Shadow area distribution analysis. We report the ratio between the shadow regions and the whole images in our complex shadow dataset, ISTD dataset~\cite{wang2018stacked}, and SBU dataset~\cite{hou2019large, vicente2016noisy, vicente2016large}. The average ratio of the whole dataset is reported in each subcaption.}
%	\label{fig:shadow_area}
%	\vspace{-1mm}
%\end{figure*}


==> section0-abstract.tex <==
\begin{abstract}

Shadow detection in general photos is a nontrivial problem, due to the complexity of the real world.
%
Though recent shadow detectors have already achieved remarkable performance on various benchmark data, their performance is still limited for general real-world situations.
%
In this work, we collected shadow images for multiple scenarios and compiled a new dataset of 10,500 shadow images, each with labeled ground-truth mask, for supporting shadow detection in the complex world.
%
Our dataset covers a rich variety of scene categories, with diverse shadow sizes, locations, contrasts, and types.
%
Further, we comprehensively analyze the complexity of the dataset, 
present a fast shadow detection network with a detail enhancement module to harvest shadow details, 
and demonstrate the effectiveness of our method to detect shadows in general situations.

%Further, we design the fast shadow detection network (FSDNet), formulate the detail enhancement module to help discover shadow boundaries and tiny shadows, and demonstrate the effectiveness of FSDNet to detect shadows in various real-world situations.
%
%Experimental results on our benchmark dataset show that FSDNet performs favorably against the state-of-the-art methods with the fastest speed and the least network parameters.


%Shadow detection in real-world photos is a very complicated problem.
%, since there may exist multiple shadows cast by multiple objects and lights and the shadows may also lie on or go across multiple background objects.
%
%Although the recent shadow detection algorithms have achieved remarkable performance on the current benchmark datasets, their performance is still limited under various types of real-world situations.
%The existing shadow detection datasets contain mainly shadows cast by single or few separate objects, which do not model the complexity of the real world.
%
%In this paper, we prepare a new benchmark dataset, which contains $10,500$ shadow images with well-labeled ground-truth masks, to support shadow detection for a complex world.
%
%This dataset includes a rich variety of scene categories, diverse proportions of shadow areas, separated shadows, and shadow locations, as well as lower color contrast between shadow and non-shadow regions. 
%
%Furthermore, we design a fast shadow detection network (FSDNet) by first adopting a direction-aware spatial context module to aggregate global information and then formulating a detail enhancement module to discover shadow details.
%
%We perform various experiments on our benchmark dataset by comparing our network with recent methods and our network. 
%Experimental results on our benchmark dataset show that FSDNet 
%performs favorably against the state-of-the-art methods with the fastest speed and the least network parameters.
%in terms of accuracy and speed with only $4M$ network parameters.



%Recent shadow detection algorithms have achieved remarkable performance on various benchmark datasets, which 
%
%These datasets do not adequately model the complexity of shadows in the real-world
%In this paper, we prepare new dataset to support the
%detection of complex shadows in several different real situations. 
%Recent deep learning techniques for shadow detection have achieved remarkable performance on various benchmark datasets, which contains mainly shadows cast by single or few separate objects. 
%shadow detection in the complex real-world photos is still challenging


 

%Deep learning techniques for point cloud data have demonstrated great potentials in solving classical problems in 3D computer vision such as 3D object classification and segmentation. Several recent 3D object classification methods have reported state-of-the-art performance on CAD model datasets such as ModelNet40 with high accuracy (∼92\%). Despite such impressive results, in this paper, we argue that object classification is still a challenging task when objects are framed with real-world settings. To prove this, we introduce ScanObjectNN, a new real-world point cloud object dataset based on scanned indoor scene data. From our comprehensive benchmark, we show that our dataset poses great challenges to existing point cloud classification techniques as objects from real-world scans are often cluttered with background and/or are partial due to occlusions. We identify three key open problems for point cloud object classification, and propose new point cloud classification neural networks that achieve state-of-the-art performance on classifying objects with cluttered background. Our dataset and code are publicly available in our project page.

\end{abstract}




==> table_CUHK_comparision_val.tex <==
\begin{table*}  [tp]
	\begin{center}
		\caption{Comparison with the state-of-the-art methods on the val set of our shadow dataset in terms of $F_\beta^\omega$ and BER. All of the methods were trained on the training set of our shadow dataset and did not use any post-processing method, \eg, CRF.}
		\label{table:rain100H}
		%\vspace*{-2mm}
	%	\resizebox{1.0\linewidth}{!}{%
			\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
				\hline
				%\multirow{2}{*}{Method} &  \multicolumn{6}{c|}{Val} & \multicolumn{6}{c|}{Test} \\
			    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Overall} & \multicolumn{2}{c|}{shadow-ADE}& \multicolumn{2}{c|}{shadow-KITTI} & \multicolumn{2}{c|}{shadow-MAP} & \multicolumn{2}{c|}{shadow-USR} & \multicolumn{2}{c}{shadow-WEB}  \\
			    
			    \cline{2-13}
			    & $F_\beta^\omega$ & BER & $F_\beta^\omega$ & BER & $F_\beta^\omega$ & BER & $F_\beta^\omega$ & BER & $F_\beta^\omega$ & BER & $F_\beta^\omega$ & BER \\
	
				\hline
				\hline
				
				DSDNet~\cite{zheng2019distraction} & 82.35 & 9.64 & 
				72.16 & 12.97 &
				85.90 & 7.89 &
				80.55 & 9.08 &
				85.58 & 4.33 &
				81.04 & 7.95  \\
				
				%\hline
				
				BDRAR~\cite{zhu2018bidirectional}& 83.32 & 10.14 &
				74.04 & 12.70 &
				84.50 & 9.76 &
				81.44 & 10.10 &
				88.47 & 4.96 &
				82.41 & 9.24 \\
				
				%\hline
				
								
				A+D Net~\cite{le2018a+d}& 82.98 & 12.53 & 
				72.87 & 16.69 &
				88.69 & 8.61 &
				80.11 & 13.12 & 
				84.94 & 6.74 &
				81.18 & 13.32  \\
				
				%\hline
				
				DSC~\cite{hu2019direction,Hu_2018_CVPR}& 81.11 & 9.43 &  
				71.22 & 12.06 &  
				84.96 & 7.63 & 
				78.35 & 9.69 & 
				84.31 & 4.83 & 
				79.94 & 9.33 \\
				
				\hline
				
		
		
				
				

				
			\end{tabular} %}
	\end{center}
	%\vspace{-4mm}
\end{table*}
